Agnostic Learning of General ReLU Activation Using Gradient Descent

We provide a convergence analysis of gradient descent for the problem of agnostically learning a single ReLU function with moderate bias under Gaussian distributions. Unlike prior work that studies the setting of zero bias, we consider the more challenging scenario when the bias of the ReLU function is non-zero. Our main result establishes that starting from random initialization, in a polynomial number of iterations gradient descent outputs, with high probability, a ReLU function that achieves an error that is within a constant factor of the optimal error of the best ReLU function with moderate bias. We also provide finite sample guarantees, and these techniques generalize to a broader class of marginal distributions beyond Gaussians.

==> results.tex <==
We now provide an overview of our analysis. For complete proofs of the lemmas and propositions, please refer to the supplementary material (Appendix~\ref{app:proofs}).

Recall that our goal throughout the learning process is to find a $w \in \R^{d+1}$ such that $L(w)$ achieves a comparable performance to $OPT = L(v)$. In order to accomplish this, we aim to find $w$ such that it is close to $v$, i.e. $\|w - v\|$ is small. Note that approximating $v$ suffices to achieve an error close to $OPT$, since we can upper-bound $L(w)$ as

%\anote{Doesn't the loss function have a factor of 1/2?}
\begin{equation*}
    L(w) =~ \dfrac{1}{2} \E \Big[ (\sigma(w^\top x) - y)^2 \Big]
    =~ \dfrac{1}{2} \E \Big[ (\sigma(w^\top x) - \sigma(v^\top x) + \sigma(v^\top x) - y)^2 \Big]
\end{equation*}
\begin{equation*}
    \leq~ 2 \cdot \dfrac{1}{2} \E \Big[ (\sigma(w^\top x) - \sigma(v^\top x))^2 \Big] + 2 \cdot \dfrac{1}{2} \E \Big[ (\sigma(v^\top x) - y)^2 \Big]
    =~ 2F(w) + 2OPT
\end{equation*}
through Young's inequality. The realizable portion of the loss $F(w)$ becomes $O(OPT)$ when $\norm{w-v} \le O(\sqrt{OPT})$ (see Lemma~\ref{lem:f-lipschitz} for a proof), and as a consequence we will get $O(OPT)$ error in total. 

To formalize our intuition above, we adapt a similar proof strategy used in \cite{frei2020agnostic}. Namely, we argue that when optimizing with respect to the agnostic loss $L(w_t)$, we are always making some non-trivial progress due to a decrease in $\norm{w_t-v}$ and due to a decrease in $F(w_t)$ (which is just the realizable portion of the loss). Moreover, whenever we stop making progress, we will argue that at this point either $\norm{w_t-v} \le O(\sqrt{OPT})$ or $\norm{\nabla F(w_t)} \le O(\sqrt{OPT})$; in both cases, this iterate already achieves an error of $O(OPT)$ due to Lemma~\ref{lem:f-lipschitz} and Lemma~\ref{lem:grad-opt}.

\paragraph{Challenges in arguing progress. } Unlike \cite{frei2020agnostic} which only considers ReLU neurons with zero bias, allowing non-zero bias terms imposes extra technical challenges. For example, the probability measure of $\{w^\top x \geq 0, v^\top x \geq 0\}$ under Gaussian distributions, which is vital to deriving the gain in each gradient descent step, does not have a closed-form expression when bias is present. Furthermore we cannot afford to lose any dimension dependent factors or assume boundedness. Thus, to address these difficulties, more detailed analyses (e.g. Lemma \ref{lem:jointprob}, \ref{lem:inner-product-lb}) are needed to facilitate our argument.

On the other hand, tackling non-zero bias terms requires additional assumptions when initializing $w_0$ as well. In our analysis, we assume that $w_0$ is initialized such that $F(w_0)$ is strictly less than $F(0)$ by a constant amount $\delta>0$ (this is inspired by \cite{vardi2021learning}, however $\delta$ can be inverse-polynomially small in their case). This is guaranteed with constant probability by our choice of initialization in Section~\ref{sec:init}. The high-level intuition behind such assumption is to ensure that gradient descent does not get trapped around a highly non-smooth region (e.g. when $w = 0$) by making it start at somewhere better than it, so that $w$ keeps moving closer to $v$.
Despite the same assumption, it is more challenging to implement it in our case (Lemma~\ref{lem:grad-opt}) because of the agnostic setting. % emphasize that utilizing it in our works requires extra analysis. 
This is because \cite{vardi2021learning} heavily relies on the realizability assumption to simplify its analysis. %As a consequence, we established extra results (Lemma \ref{lem:grad-opt}) to incorporate it under the agnostic setting.

We also highlight our improvements on the dependency of the dimension $d$. In previous works, the guarantees of  the algorithm has a dependence on $d$ either explicitly or implicitly. For instance, in \cite{frei2020agnostic} the $O(\sqrt{OPT})$ guarantee for ReLU neurons includes a coefficient in terms of $B_X$ (the upper-bound for $\|x\|$), which for Gaussian inputs is in fact $\sqrt{d}$; or for example in \cite{vardi2021learning}, the gain for each gradient descent iteration $\gamma$ comes with a dependency on $c$ (the upper-bound for $\|x\|$) of $c^{-8}$, which for Gaussian is $d^{-4}$. In contrast, we avoid such dependencies on the dimension $d$ in order to obtain our guarantees.


We first establish two important lemmas we will later utilize in proving progress in each iteration. As stated in the preliminaries, we assume in the rest of the section that $\norm{\tv}_2=1$. The first lemma gives a lower bound on the measure of the region where both $\sigma(v^\top x)$ and $\sigma(w_t^\top x)$ are non-zero. 
Our inductive hypotheses will ensure that this lower bound is a constant (if $|b_v|$ is a constant). 
\begin{restatable}[Lower bound on the measure of the intersection]{lemma}{jointprob}
\label{lem:jointprob}
\label{lem:gen:jointprob}
Suppose the marginal distribution $\tcDx$ over $\tx$ is $O(1)$-regular. There exists an absolute constant $c>0$ such that for all $\delta>0$, if $F(w) \leq F(0) - \delta$ then 
\begin{equation}\label{eq:jointprob}
    \Pr[w^\top x \geq 0, v^\top x \geq 0] \geq \frac{\delta^2}{c\norm{w}_2^4 \norm{v}_2^4} = \frac{\delta^2}{c\norm{w}_2^4 (1+|b_v|^2)^2}.
\end{equation}
\end{restatable}


With Lemma \ref{lem:jointprob}, the following lemma allows us to get an improvement on the realizable portion of the loss function as long as the gradient is non-negligible. We state and prove this lemma for the general case of $O(1)$-regular marginal distributions. 

%We now give a generalization of Lemma~\ref{lem:inner-product-lb} that generalizes to $O(1)$-regular distributions.
\begin{restatable}[Improvement from the first order term]{lemma}{innerproductlb}
 \label{lem:inner-product-lb}
%\begin{lemma}[Improvement from the first order term]
\label{lem:gen:inner-product-lb}
Suppose the marginal over $\tx$ is $O(1)$-regular. There exists absolute constants $c_1, c_2 > 0$ such that for any $\delta>0$, if $\norm{v}_2, \norm{w}_2 \le B$ and $F(w) \leq F(0) - \delta$ then 
\begin{equation}
    \langle \nabla F(w), w-v \rangle \geq  \gamma  \|w-v\|^2, \text{ where } \gamma = \frac{c_1 \delta^9}{B^{28}}.
\end{equation}
\end{restatable}
The constants $c_1, c_2$ depend on the constants $\beta_1, \beta'_2, \beta_2, \beta_4$ etc. in the regularity assumption of $\tcDx$. 
We remark that for our setting of parameters $\delta = \Omega(1)$ and $B=O(1)$, and hence we will conclude that $\iprod{\nabla F, w-v} \ge \Omega( \norm{w-v}_2^2)$. 

\begin{proof}
This lemma only concerns the ``realizable portion'' of the loss function $F(w)$. 

Let $u=(\tu, b_u) \in \R^{d+1}$ be the unit vector along $w-v$. We have
\begin{align}
    \iprod{\nabla F(w), w-v} & = \E\Big[ \big(\sigma(w^\top x) - \sigma(v^\top x)\big) \sigma'(w^\top x) (w^\top x - v^\top x)\Big] \nonumber \\
    &= \E\Big[ \big(w^\top x - v^\top x\big)^2 \mathbf{1}[w^\top x \ge 0,  v^\top x \ge 0]\Big] \nonumber\\
    &\qquad + \E\Big[ w^\top x \big(w^\top x - v^\top x \big)  \mathbf{1}[w^\top x \ge 0,  v^\top x < 0] \Big]\nonumber \\
    &\ge  \E\Big[ \big(w^\top x - v^\top x\big)^2 \mathbf{1}[w^\top x \ge 0,  v^\top x \ge 0]\Big] \nonumber\\
    &= \norm{w-v}_2^2 \cdot \E\Big[ (u^\top x)^2  \mathbf{1}[w^\top x \ge 0,  v^\top x \ge 0]\Big] \label{eq:in-lb:temp1}
\end{align}

Let $q \coloneqq c \delta^2 / B^8 $ and $\tau \coloneqq c' \frac{\delta^4}{B^{16} }$ for some sufficiently small absolute constant $c'>0$ that will be chosen later. 
We will now lower bound the contribution from just the samples that achieve a value $(u^\top x)^2 > \tau^2$ using Lemma~\ref{lem:jointprob}, that lower bounds $\Pr[w^\top x \ge 0, v^\top x \ge 0] \ge c \delta^2/ B^8=q$:
\begin{align}
&\E\Big[ (u^\top x)^2  \mathbf{1}[w^\top x \ge 0,  v^\top x \ge 0]\Big]  \nonumber \\
&\ge \tau^2 \cdot \Pr_x \Big[ w^\top x \ge 0,  v^\top x \ge 0, (u^\top x)^2 \ge \tau^2 \Big] \nonumber\\
&\ge \tau^2 \cdot \Big(\Pr_x \big[ w^\top x \ge 0,  v^\top x \ge 0 \big] - \Pr_x\big[ (u^\top x)^2 < \tau^2 \big] \Big) \nonumber\\
&\ge \tau^2 \cdot \Big( q - \Pr_{\tx \sim N(0,I)}[|\tu^\top x+b_u|< \tau] \Big). \label{eq:in-lb:temp2}
\end{align}
Now we just need to upper bound $\Pr_{\tx}[|\tu^\top \tx + b_u| < \tau]$.  Let $\beta = \norm{\tu}_2$. %Note that $\tu^\top \tx \sim \mathcal{N}(0, \beta^2)$.  
If $\beta=\norm{\tu}_2 \ll |b_u|$, then $|b_u|$ is itself large, and $\tu^\top \tx$ is too small in comparison to bring down $|\tu^\top \tx + b_u|$. On the other hand, if $\beta = \norm{\tu}_2$ is not too small, then the anti-concentration (or spread out density) of the distribution $\tcDx$ ensures that $|\tu^\top \tx + b_u|$ is small with very low probability. We now formalize this intuition.  

Suppose $\beta = \norm{\tu}_2  \le \tfrac{1}{4\beta_4}(q/2)^{1/4}$. Then $|b_u|>1/2$, since $\norm{u}_2=1$. Also from our choice, $\tau< 1/4$.  Hence by the bounded fourth moments property of $\tcDx$ and Markov's inequality,
$$ \Pr_{\tx \sim \tcDx}[ |\tu^\top \tx + b_u|< \tau ] \le \Pr_{\tx \sim \tcDx}[ |\tu^\top \tx| > \tfrac{1}{4} ] \le \frac{\E_{\tx \sim \tcDx}[\iprod{\tu,\tx}^4]}{(1/4)^4} \le \beta_4 (4\norm{\tu}_2)^4 \le \frac{q}{2}. $$

On the other hand, if $\beta = \norm{\tu}_2 > \tfrac{1}{4 \beta_4}(q/2)^{1/4}$. Suppose $\hat{u}$ is the unit vector along $\tu$. Then using the fact that $\hat{u}^\top \tx = \tu^\top \tx / \norm{\tu}$ is anti-concentrated by the properties of $\tcDx$. Hence we have for some  constant $\beta_3>0$
\begin{align*}
    \Pr_{\tx \sim \tcDx}\Big[ |\tu^\top \tx + b_u|< \tau \Big] &= \Pr_{\tx \sim \tcDx}\Big[ \hat{u}^\top \tx \in ( \tfrac{b_u-\tau}{\norm{\tu}} - \tfrac{b_u+\tau}{\norm{\tu}}) \Big] \le \frac{\beta_3 \tau}{\norm{\tu}} \le 32\beta_3 \beta_4 \Big(\frac{2}{q}\Big)^{1/4} \tau  < \frac{q}{2},
\end{align*}
from our choice of parameters since $\tau = c' \delta^{5/2}/(B^{10} \beta_3 \beta_4)$ for a sufficiently small $c'>0$. Substituting back in \eqref{eq:in-lb:temp2} and \eqref{eq:in-lb:temp1} we have
$$ \iprod{\nabla F(w), w-v} \ge \tau^2 \cdot \frac{q}{2} \ge c_1 \norm{w-v}_2^2 \cdot \frac{\delta^5 }{B^{20} \beta_3^2 \beta_4^2} \cdot \frac{\delta^2}{B^8} \ge c_1 \norm{w-v}_2^2 \cdot \frac{\delta^9}{B^{28}}.$$
\end{proof}



% \begin{restatable}[Improvement from the first order term]{lemma}{innerproductlb}
% \label{lem:inner-product-lb}
% There exists absolute constants $c_1, c_2 > 0$ such that for any $\delta>0$, if $\norm{v}_2, \norm{w}_2 \le B$ \anote{should we use a different symbol instead of $B$?} and $F(w) \leq F(0) - \delta$ then 
% \begin{equation}
%     \langle \nabla F(w), w-v \rangle \geq  \gamma  \|w-v\|^2, \text{ where } \gamma = \frac{c_1 \delta^7}{B^{25}}.
% \end{equation}
% \end{restatable}
% We remark that for our setting of parameters $\delta = \Omega(1)$ and $B=O(1)$, and hence we will conclude that $\iprod{\nabla F, w-v} \ge \Omega( \norm{w-v}_2^2)$. 

% \begin{proof}
% This lemma only concerns the ``realizable portion'' of the loss function $F(w)$. We follow the same proof outline from \cite{vardi2021learning}, while being careful to ensure that there are no dimension dependent terms, especially dependence on $\norm{x}$ (which are themselves $\sqrt{d}$). 

% Let $u=(\tu, b_u) \in \R^{d+1}$ be the unit vector along $w-v$. We have
% \begin{align}
%     \iprod{\nabla F(w), w-v} & = \E\Big[ \big(\sigma(w^\top x) - \sigma(v^\top x)\big) \sigma'(w^\top x) (w^\top x - v^\top x)\Big] \nonumber \\
%     &= \E\Big[ \big(w^\top x - v^\top x\big)^2 \mathbf{1}[w^\top x \ge 0,  v^\top x \ge 0]\Big] \nonumber\\
%     &\qquad + \E\Big[ w^\top x \big(w^\top x - v^\top x \big)  \mathbf{1}[w^\top x \ge 0,  v^\top x < 0] \Big]\nonumber 
% \end{align}
% \begin{align}
% \iprod{\nabla F(w), w-v}     &\ge  \E\Big[ \big(w^\top x - v^\top x\big)^2 \mathbf{1}[w^\top x \ge 0,  v^\top x \ge 0]\Big] \nonumber\\
%     &= \norm{w-v}_2^2 \cdot \E\Big[ (u^\top x)^2  \mathbf{1}[w^\top x \ge 0,  v^\top x \ge 0]\Big] \label{eq:in-lb:temp1}
% \end{align}

% Let $q \coloneqq c \delta^2 / B^8 $ and $\tau \coloneqq c' \frac{\delta^2}{B^8 \sqrt{\log (B/\delta)}}$ for some sufficiently small absolute constant $c'>0$ that will be chosen later. 
% We will now lower bound the contribution from just the samples that achieve a value $(u^\top x)^2 > \tau^2$ using Lemma~\ref{lem:jointprob} that lower bounds $\Pr[w^\top x \ge 0, v^\top x \ge 0] \ge c \delta^2/ B^8=q$ as
% \begin{align}
% &\E\Big[ (u^\top x)^2  \mathbf{1}[w^\top x \ge 0,  v^\top x \ge 0]\Big]  \nonumber \\
% &\ge \tau^2 \cdot \Pr_x \Big[ w^\top x \ge 0,  v^\top x \ge 0, (u^\top x)^2 \ge \tau^2 \Big] \nonumber\\
% &\ge \tau^2 \cdot \Big(\Pr_x \big[ w^\top x \ge 0,  v^\top x \ge 0 \big] - \Pr_x\big[ (u^\top x)^2 < \tau^2 \big] \Big) \nonumber\\
% &\ge \tau^2 \cdot \Big( q - \Pr_{\tx \sim N(0,I)}[|\tu^\top x+b_u|< \tau] \Big). \label{eq:in-lb:temp2}
% \end{align}
% Now we just need to upper bound $\Pr_{\tx}[|\tu^\top \tx + b_u| < \tau]$.  Let $\beta = \norm{\tu}_2$. Note that $\tu^\top \tx \sim \mathcal{N}(0, \beta^2)$.  If $\beta=\norm{\tu}_2 \ll |b_u|$, then $|b_u|$ is itself large, and $\tu^\top \tx$ is too small in comparison to bring down $|\tu^\top \tx + b_u|$. On the other hand, if $\beta = \norm{\tu}_2$ is not too small, then the spread out probability density ensures that $|\tu^\top \tx + b_u|$ is small with very low probability. We now formalize this intuition.  

% Suppose $\beta = \norm{\tu}_2  < \tfrac{1}{8\sqrt{\log(2/q)}}$. Then $|b_u|>1/2$, as $\norm{u}_2=1$, and  by choice, $\tau< 1/4$, so
% $$ \Pr_{\tx \sim N(0,I)}[ |\tu^\top \tx + b_u|< \tau ] \le \Pr_{\tx \sim N(0,I)}[ |\tu^\top \tx| > \tfrac{1}{4} ] = \Pr_{g \sim N(0,\beta^2)}[ |g|> \tfrac{1}{4} ] \le \frac{q}{2}. $$

% On the other hand, if $\beta = \norm{\tu}_2 > \tfrac{1}{8\sqrt{\log(2/q)}}$. Then using the fact that $\tu^\top \tx \sim \mathcal{N}(0,\beta^2)$ and the anti-concentration (or small-ball probability) we have for some absolute constant $c_3>0$
% \begin{align*}
%     \Pr_{\tx \sim N(0,I)}\Big[ |\tu^\top \tx + b_u|< \tau \Big] &= \Pr_{g \sim N(0,\beta^2)}\Big[ g \in ( b_u - \tau, b_u+\tau) \Big] \le \frac{c_3 \tau}{\beta} \le 8c_3 \tau \sqrt{\log (2/q)} < \frac{q}{2},
% \end{align*}
% from our choice of parameters since $\tau = c'\delta^2/(B^8 \sqrt{\log(B/\delta)})$ for a sufficiently small $c'>0$. Substituting back in \eqref{eq:in-lb:temp2} and \eqref{eq:in-lb:temp1} we have
% $$ \iprod{\nabla F(w), w-v} \ge c_1 \norm{w-v}_2^2 \cdot \frac{\delta^4 }{B^16 \log(B/\delta)} \cdot \frac{\delta^2}{B^8} \ge c_1 \norm{w-v}_2^2 \cdot \frac{\delta^7}{B^{25}}.$$
% We remark that this analysis also goes through with slightly weaker parameters under milder assumptions (like bounded fourth-moment instead of sub-Gaussianity). 
% \end{proof}


\subsection{Main proof strategy} \label{sec:strategy}
With these two key lemmas, we are now ready to discuss the proof overview of the main theorem (Theorem~\ref{thm:main-informal}). 
%We now present the main technical details of our analysis. 
We inductively maintain two invariants in every iteration of the algorithm:
\[ \text{(A)}~~~ \norm{w_t -v}_2 \le O(1),~~~~\text{ and } ~~~\text{(B)}~~ F(0) - F(w_t) = \Omega(1). \label{eq:invariants}\]
These two invariants are true at $t=0$ due to our initialization $w_0$. Lemma~\ref{lem:init} guarantees with at least constant probability $\Omega(1)$, both the invariants hold for $w_0$. 
% \anote{proposition statement needs to rewritten. }
% \begin{restatable}[]{proposition}{mainprop}
% Assume $w_0$ is initialized such that $F(w_0) \leq F(0) - \delta$ for some $\delta > 0$ and $\|w_t - v\| \leq B_{wv}$ for all $t$, then gradient descent run on the agnostic loss $L(w_t)$ in $T \leq O(\eta^{-1} OPT^{-1})$ timesteps finds $w_T$ such that $F(w_T) \leq O(\gamma^{-c_2} OPT)$ with learning rate $\eta \leq O(d^{-1})$.
% \end{restatable}
The proof that both the invariants continue to hold follows from the progress made by the algorithm due to a decrease in both $\norm{w_t-v}_2$ and $F(w_t)$ (note that we only need to show they do not increase to maintain the invariant). 

The argument consists of two parts.
First, assuming $F(w_t) \leq F(0) - \delta$ holds (for some constant $\delta>0$), we establish that whenever $\|w_t-v\|^2 > \gamma OPT$ for some constant $\gamma > 0$, gradient descent always makes progress i.e. $\|w_t - v\|^2 - \|w_{t+1} - v\|^2$ is lower bounded. 
Next, we argue that if $w_0$ is initialized such that $F(w_0) \leq F(0) - \delta$ for some constant $\delta > 0$, then throughout gradient descent $F(w_t)$ always decreases, i.e. the inequality $F(w_t) \leq F(w_0) \leq F(0) - \delta$ always holds.

However, unlike \cite{vardi2021learning} where they focus on the realizable setting, analyzing gradient descent on the agnostic loss $L(w)$ is more challenging, since the update depends on $\nabla L(w)$ and not $\nabla F(w)$. In fact, the additional term from the ``non-realizable'' portion of the loss $L(w)$ can overwhelm the contribution from the realizable loss when either $\norm{\nabla F}_2 \le O(\sqrt{OPT})$ or $\norm{w_t - v}_2 \le O(\sqrt{OPT})$. The following two lemmas argue that in both of these cases, the current iterate already achieves $O(OPT)$ error (and this iterate will be the $T$ that satisfies the guarantee of Theorem~\ref{thm:main-informal}). 

\begin{restatable}[Success if $\norm{\nabla F} \le O(\sqrt{OPT})$]{lemma}{gradopt}
\label{lem:grad-opt}
Suppose $B , \delta>0$ are constants such that $\norm{v}_2, \norm{w}_2 \le B$ and $F(w) \leq F(0) - \delta$. Then there exists a constant $C_G>0$, such that if $\|\nabla F(w)\| \leq C_G \sqrt{OPT}$ then $\|w-v\|_2 \leq O(\sqrt{OPT})$.
\end{restatable}
\begin{proof}
We can first apply Lemma \ref{lem:inner-product-lb} to conclude that
\begin{equation*}
    \langle \nabla F(w), w - v \rangle \geq~ \gamma \|w - v\|^2,
\end{equation*}
for some constant $\gamma>0$ (since $B, \delta>0$ are constants). Hence
\begin{equation*}
    \|\nabla F(w)\| \|w - v\| \geq~ \langle \nabla F(w), w - v \rangle \geq~ \gamma \|w - v\|^2, 
\end{equation*}
Thus $\norm{w-v}_2  = O(\sqrt{OPT})$
% Hence 
% \begin{equation*}
%     \Longrightarrow~ \|\nabla F(w)\| \geq~ c_1\gamma^{c_2} \|w - v\| \geq~ c_1 C_p \gamma^{c_2/2} \sqrt{OPT}
% \end{equation*}
which implies the lemma.
\end{proof}

We now argue that if $\|w_t - v\| \leq O(\sqrt{OPT})$, then $F(w_t) \leq O(OPT)$ through the following lemma; this is stated and proven for $O(1)$-regular distributions.

\begin{restatable}[Small $\|w_t - v\|$ implies small $F(w_t)$]{lemma}{flipschitz}
\label{lem:f-lipschitz}
% If $\|w_t - v\|_2 \leq O(\sqrt{OPT})$, then $F(w_t) \leq O(OPT)$.
% \end{restatable}
% \begin{lemma}[Small $\|w_t - v\|$ implies small $F(w_t)$]
\label{lem:f-lipschitz-regular}
Assume $\widetilde{\mathcal{D}}_x$ is $O(1)$-regular with parameters defined above. If $\|w_t - v\|_2 \leq O(\sqrt{OPT + \eps})$ for some $\eps > 0$, then $F(w_t) \leq O(OPT + \eps)$.
\end{restatable}
\begin{proof}
Since ReLU function is 1-Lipschitz (i.e. $|\sigma(z) - \sigma(z')| \leq |z - z'|$),
\begin{equation*}
    F(w_t) = \dfrac{1}{2} \E \Big[ (\sigma(w_t^\top x) - \sigma(v^\top x))^2 \Big]
    \leq~ \dfrac{1}{2} \E \Big[ (w_t^\top x - v^\top x)^2 \Big]
    =~ \dfrac{\|w_t - v\|^2}{2} \E \Big[ (u^\top x)^2 \Big]
\end{equation*}

where we defined $u = \frac{w_t - v}{\|w_t - v\|}$, hence the last equation. 
Now, notice by using Young's inequality, we get
\begin{equation*}
    \E \Big[ (u^\top x)^2 \Big] =~ \E \Big[ (\widetilde{u}^\top \widetilde{x} + b_u)^2 \Big]
    \leq~ 2\E \Big[ (\widetilde{u}^\top \widetilde{x})^2 \Big] + 2b_u^2
    \leq~ 2\beta_2 + 2b_u^2 \leq~ O(1)
\end{equation*}
due to the regularity assumption on $\widetilde{\mathcal{D}}_x$. Hence
\begin{equation*}
    F(w_t) \leq~ \dfrac{\|w_t - v\|^2}{2} \cdot O(1) 
    \leq~ O(\|w_t - v\|_2^2) 
    \leq~ O(OPT + \eps)
\end{equation*}
which concludes the proof.
\end{proof}






% \begin{proof}
% Observe that from the properties of the ReLU function,
% \begin{equation*}
%     F(w_t) = \dfrac{1}{2} \E \Big[ (\sigma(w_t^\top x) - \sigma(v^\top x))^2 \Big]
%     \leq~ \dfrac{1}{2} \E \Big[ (w_t^\top x - v^\top x)^2 \Big]
%     =~ \dfrac{\|w_t - v\|^2}{2} \E \Big[ (u^\top x)^2 \Big]
% \end{equation*}
% % where the first $\leq$ is due to Lipschitzness of $\sigma(\cdot)$:
% % \begin{equation*}
% %     \dfrac{|\sigma(z_1) - \sigma(z_2)|}{|z_1 - z_2|} \leq~ 1
% % \end{equation*}
% %
% %for any $z_1, z_2 \in \R$. 
% We also defined $u = \frac{w_t - v}{\|w_t - v\|}$, hence the last equation. 
% Now, notice by using Young's inequality, we get
% \begin{equation*}
%     \E \Big[ (u^\top x)^2 \Big] =~ \E \Big[ (\widetilde{u}^\top \widetilde{x} + b_u)^2 \Big]
%     \leq~ 2\E \Big[ (\widetilde{u}^\top \widetilde{x})^2 \Big] + 2b_u^2
%     =~ 2\|\widetilde{u}\|^2 + 2b_u^2 =~ 2
% \end{equation*}
% due to standard properties of Gaussian distributions. Hence
% \begin{equation*}
%     F(w_t) \leq~ \dfrac{\|w_t - v\|^2}{2} \cdot 2 =~ \|w_t - v\|^2 = O(OPT)
% \end{equation*}
% which concludes the proof.
% \end{proof}

\paragraph{Proving progress in $\norm{w_t -v}$ and $F(w_t)$.}

To show $\norm{w_t-v}$ decreases, we establish the following lemma. 

\begin{restatable}[]{lemma}{induction}
\label{lem:induction}
Assume at time $t$, $F(w_t) \leq F(0) - \delta$ where $\delta > 0$ is a constant. For some constants $C,C' > 0$, if $\|w_t - v\|^2 \geq C \cdot OPT$, then $\|w_{t+1} - v\|^2 \leq \|w_t - v\|^2 - C' \cdot OPT$.
\end{restatable}

Lemma \ref{lem:induction} is a direct consequence of the following inductive statement: for every $t$, either (a) $\|w_t - v\|^2 - \|w_{t+1} - v\|^2 \geq  C \eta OPT$ is true for some constant $C > 0$ or (b) $\|w_t - v\|^2 \leq O(\gamma^{-1} OPT)$ holds. Observe that when (b) holds Lemma~\ref{lem:f-lipschitz} implies the loss is $O(OPT)$; hence we need only assume at time $t$ (b) does not hold yet, thus it suffices focusing on showing (a) is true.

Additionally, note at each timestep $t$,
\begin{align}
    w_{t+1} &= w_t - \eta \nabla L(w_t)\\
     w_{t+1} - v &= w_t - v - \eta\nabla L(w_t)\\
    \Longrightarrow~ \|w_t - v\|^2 - \|w_{t+1} - v\|^2 &= 2\eta \langle \nabla L(w_t), w_t - v \rangle - \eta^2 \|\nabla L(w_t)\|^2.
\end{align}

Therefore, to lower-bound $\|w_t - v\|^2 - \|w_{t+1} - v\|^2$, we will give a lower bound for $\langle \nabla L(w_t), w_t - v \rangle$ and an upper bound for $\|\nabla L(w_t)\|^2$.

To show that $F(w_t)$ decreases we show that at time $t$, if gradient descent continues to make progress towards $v$, then $F(w_{t+1}) \leq F(w_t) \le F(0) - \delta$. 

We can use as a black box two lemmas given in \cite{vardi2021learning} that uses the smoothness of the function to upper bound the contribution from the second order term. 

\begin{restatable}[Lemma D.4 in \cite{vardi2021learning}]{lemma}{smooth}
\label{lem:smooth}
For any $w, w' \in \R^{d+1}$, if $~\forall \lambda \in [0,1]$ there exists constants $C_\ell, C_u > 0$ such that $\|(1-\lambda)w + \lambda w'\| \in [C_\ell, C_u]$, then $\| \nabla F(w) - \nabla F(w') \| \leq d \cdot (1+\frac{8(C_u+1)c'd}{C_{\ell}}) \|w - w'\|$ for some constant $c' > 0$.
\end{restatable}

\begin{restatable}[Lemma D.5 in \cite{vardi2021learning}]{lemma}{smoothexpansion}
\label{lem:smooth-expansion}
Let $f: \R^{d+1} \to \R$ and $\ell > 0$. Assume for any $w, w' \in \R^{d+1}$ such that $\forall~ \lambda \in [0,1]$

\[
    \|\nabla f((1-\lambda)w + \lambda w') - \nabla f(w)\| \leq \ell\lambda \|w' - w\|
\]

then the following holds:
\[
    f(w') \leq f(w) + \langle \nabla f(w), w' - w \rangle + \dfrac{\ell}{2}\|w' - w\|^2
\]

\end{restatable}

These two lemmas are used to get a non-trivial bound on the second order term. The progress in $F(w)$ follows crucially relies on Lemma~\ref{lem:inner-product-lb} that was proven earlier. Please see Appendix~\ref{app:proofs} in the supplementary material for the detailed proofs. 


%\paragraph{Putting it together.}
